SatDepth: A Novel Dataset for Satellite Image Matching

Recent advances in deep-learning based methods for image matching have demonstrated their superiority over traditional algorithms, enabling correspondence estimation in challenging scenes with significant differences in viewing angles, illumination and weather conditions. However, the existing datasets, learning frameworks, and evaluation metrics for the deep-learning based methods are limited to ground-based images recorded with pinhole cameras and have not been explored for satellite images. In this paper, we present ``SatDepth'', a novel dataset that provides dense ground-truth correspondences for training image matching frameworks meant specifically for satellite images. Satellites capture images from various viewing angles and tracks through multiple revisits over a region. To manage this variability, we propose a dataset balancing strategy through a novel image rotation augmentation procedure. This procedure allows for the discovery of corresponding pixels even in the presence of large rotational differences between the images. We benchmark four existing image matching frameworks using our dataset and carry out an ablation study that confirms that the models trained with our dataset with rotation augmentation outperform (up to 40% increase in precision) the models trained with other datasets, especially when there exist large rotational differences between the images.

==> caps_angle_performance_all_aois.tex <==

\begin{minipage}{0.02\linewidth}
    \hfill
\end{minipage}
\hfill\hfill
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{Jacksonville}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{San Fernando}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{Omaha}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{UCSD}}
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\linewidth}
\rotatebox[origin=c]{90}{View-Angle Difference}
\end{minipage}
\hfill{\vline width 1pt}\hfill
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/jacksonville/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/argentina/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/omaha/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/ucsd/average_precision_vs_intersection_angle.pdf}       
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\linewidth}
    \rotatebox[origin=c]{90}{Track-Angle Difference}
    \end{minipage}
    \hfill{\vline width 1pt}\hfill
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/jacksonville/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/argentina/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/omaha/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/caps/ucsd/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}

\vspace{1.5mm}


==> cvpr_template_preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> dualrc_angle_performance_all_aois.tex <==

\begin{minipage}{0.02\linewidth}
    \hfill
\end{minipage}
\hfill\hfill
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{Jacksonville}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{San Fernando}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{Omaha}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{UCSD}}
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\linewidth}
\rotatebox[origin=c]{90}{View-Angle Difference}
\end{minipage}
\hfill{\vline width 1pt}\hfill
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/jacksonville/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/argentina/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/omaha/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/ucsd/average_precision_vs_intersection_angle.pdf}       
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\linewidth}
    \rotatebox[origin=c]{90}{Track-Angle Difference}
    \end{minipage}
    \hfill{\vline width 1pt}\hfill
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/jacksonville/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/argentina/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/omaha/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/dualrc/ucsd/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}

\vspace{1.5mm}


==> figure_tables/matcher_performance_main.tex <==
  \begin{minipage}{0.4\linewidth}
    \centering  
      \small{
        \textbf{Patch Performance}}
  \end{minipage}
  % \hspace{1mm}
  \begin{minipage}{0.3\linewidth}
    \centering
    \small{        
        \textbf{satLoFTR on Jacksonville}
        }
  \end{minipage}
% 
  \begin{minipage}{0.3\linewidth}
    \centering  
      \small{          
          \textbf{satLoFTR on San Fernando}
          }
  \end{minipage}
  \hfill
  % ---------------------------------------------------------------------------
  \begin{minipage}{0.4\linewidth}
    \centering
    \centering
    \tiny{
    \setlength\tabcolsep{1.0pt}
  \input{tables/jax_and_argentina_matcher_performance_table.tex}
    }
  \end{minipage}
  % 
  % \hspace{1mm}
  \begin{minipage}{0.3\linewidth}
    \centering
      % \includegraphics[width=\linewidth]{images/more_plots/av_precision_jax_argentina_loftr/jacksonville/average_precision_combined}
      % simulated rot
      \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model_combined/loftr/jacksonville/average_precision_combined.pdf}    
  \end{minipage}
  % 
  \begin{minipage}{0.3\linewidth}
    \centering
    % \includegraphics[width=\linewidth]{images/more_plots/av_precision_jax_argentina_loftr/argentina/average_precision_combined}
    % simulated rot
    \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model_combined/loftr/argentina/average_precision_combined.pdf} 
  \end{minipage}
  % 
  % \hfill

==> jax_loftr_matches_table.tex <==
\begin{minipage}{0.3\textwidth}
    \centering
    \small{
        % \textbf{Large View-Intersection Angle}
        \textbf{Large View-Angle Difference}
        }
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.3\textwidth}
    \centering
    \small{
        % \textbf{Large Relative-Track Angle}
        \textbf{Large Track-Angle Difference}
        }
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.3\textwidth}
    \centering
    \small{\textbf{Large Time Difference}}
\end{minipage}

\vspace{1mm}
\begin{minipage}{0.3\textwidth}
    \includegraphics[width=\linewidth]{./images/hard_pairs/loftr/testing_set_jacksonville_144_hard_pairs_intersection/aoi_rect_piece_144_18FEB16WV031200016FEB18164007-P1BS-501504472090_01_P001_________AAE_0AAAAABPABP0_and_21DEC15WV031200015DEC21161108-P1BS-501504473080_01_P001_________AAE_0AAAAABPABG0_matches.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.3\textwidth}
    \includegraphics[width=\linewidth]{./images/hard_pairs/loftr/testing_set_jacksonville_144_hard_pairs_rel_track/aoi_rect_piece_144_11OCT14WV031100014OCT11155720-P1BS-500648061020_01_P001_________AAE_0AAAAABPABR0_and_05OCT14WV031100014OCT05160138-P1BS-500648062040_01_P001_________AAE_0AAAAABPABL0_matches.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.3\textwidth}
    \includegraphics[width=\linewidth]{./images/hard_pairs/loftr/testing_set_jacksonville_144_hard_pairs_time_diff/aoi_rect_piece_144_01NOV15WV031100015NOV01162034-P1BS-500648061060_01_P001_________AAE_0AAAAABPABE0_and_14MAY15WV031200015MAY14160906-P1BS-501504473050_01_P001_________AAE_0AAAAABPABS0_matches.pdf}       
\end{minipage}

\vspace{1.5mm}


==> loftr_angle_performance_all_aois.tex <==

\begin{minipage}{0.02\linewidth}
    \hfill
\end{minipage}
\hfill\hfill
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{Jacksonville}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{San Fernando}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{Omaha}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \centering
    \small{\textbf{UCSD}}
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\linewidth}
\rotatebox[origin=c]{90}{View-Angle Difference}
\end{minipage}
\hfill{\vline width 1pt}\hfill
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/jacksonville/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/argentina/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/omaha/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/ucsd/average_precision_vs_intersection_angle.pdf}       
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\linewidth}
    \rotatebox[origin=c]{90}{Track-Angle Difference}
    \end{minipage}
    \hfill{\vline width 1pt}\hfill
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/jacksonville/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/argentina/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/omaha/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\linewidth}
        \includegraphics[width=\linewidth]{./images/more_plots/rot_aug_ablation_per_model/loftr/ucsd/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}

\vspace{1.5mm}


==> loftr_angle_performance_all_aois_simulated_rot.tex <==

\begin{minipage}{0.02\textwidth}
    \hfill
\end{minipage}
\hfill\hfill
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \centering
    \small{\textbf{Jacksonville}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \centering
    \small{\textbf{San Fernando}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \centering
    \small{\textbf{Omaha}}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \centering
    \small{\textbf{UCSD}}
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\textwidth}
\rotatebox[origin=c]{90}{View-Angle Difference}
\end{minipage}
\hfill{\vline width 1pt}\hfill
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/jacksonville/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/argentina/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/omaha/average_precision_vs_intersection_angle.pdf}       
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.22\textwidth}
    \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/ucsd/average_precision_vs_intersection_angle.pdf}       
\end{minipage}


\vspace{1.5mm}
\begin{minipage}{0.02\textwidth}
    \rotatebox[origin=c]{90}{Track-Angle Difference}
    \end{minipage}
    \hfill{\vline width 1pt}\hfill
    \hspace{1mm}
    \begin{minipage}{0.22\textwidth}
        \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/jacksonville/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\textwidth}
        \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/argentina/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\textwidth}
        \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/omaha/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}{0.22\textwidth}
        \includegraphics[width=\linewidth]{./images/more_plots/simulated_rot_exps_per_model/loftr/ucsd/average_precision_vs_rel_track_angle.pdf}       
    \end{minipage}

\vspace{1.5mm}


==> matching_plot.tex <==
\begin{figure*}[ht!]
    \centering
    \begin{minipage}{0.02\textwidth}
        \hfill
    \end{minipage}%
    \hspace{1mm}%
    \begin{minipage}{0.3\textwidth}
        \centering
        \small{\textbf{LoFTR}}
    \end{minipage}%
    \hspace{1mm}%
    \begin{minipage}{0.3\textwidth}
        \centering
        \small{\textbf{DualRC-Net}}
    \end{minipage}%
    \hspace{1mm}%
    \begin{minipage}{0.3\textwidth}
        \centering
        \small{\textbf{SIFT + CAPS}}
    \end{minipage}%
    
    \vspace{1.5mm}
    \begin{minipage}{0.02\textwidth}
    \rotatebox[origin=c]{90}{Jacksonville}
    \end{minipage}%
    \hfill{\vline width 1pt}\hfill
    \hspace{1mm}%
    \begin{minipage}{0.3\textwidth}
        \includegraphics[width=\linewidth]{images/sample_matches}       
    \end{minipage}%
    \hspace{1mm}%
    \begin{minipage}{0.3\textwidth}
        \includegraphics[width=\linewidth]{images/sample_matches}
    \end{minipage}%
    \hspace{1mm}%
    \begin{minipage}{0.3\textwidth}
        \includegraphics[width=\linewidth]{images/sample_matches}
    \end{minipage}
    
    \vspace{1.5mm}
    \begin{minipage}{0.02\textwidth}
        \rotatebox[origin=c]{90}{San Fernando}
        \end{minipage}%
        \hfill{\vline width 1pt}\hfill
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}%
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}%
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}
    
    \vspace{1.5mm}
    \begin{minipage}{0.02\textwidth}
        \rotatebox[origin=c]{90}{Omaha}
        \end{minipage}%
        \hfill{\vline width 1pt}\hfill
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}%
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}%
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}

    \vspace{1.5mm}
    \begin{minipage}{0.02\textwidth}
        \rotatebox[origin=c]{90}{UCSD}
        \end{minipage}%
        \hfill{\vline width 1pt}\hfill
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}%
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}%
        \hspace{1mm}%
        \begin{minipage}{0.3\textwidth}
            \includegraphics[width=\linewidth]{images/sample_matches}
        \end{minipage}
    % \vspace{-.3cm}
    \caption{ Qualitative image matches. }
    \label{fig:qual_plots}
\end{figure*}

==> tables/argentina_matcher_performance_table.tex <==
\begin{tabular}{lcccccc}
    \toprule
    \multicolumn{7}{c}{\centering \textbf{San Fernando}}\\
    \midrule
    \multirow{2}{1cm}[-.4em]{Method} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Rot.\\ Aug.\end{tabular}}
    & \multicolumn{3}{c}{Pose estimation AUC $\uparrow$} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}P $\uparrow$ \\ \end{tabular}}%$\delta_{epi}\!=\!1$\end{tabular}} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}} N $\uparrow$ \\\end{tabular}}\\
    \cmidrule(lr){3-5}
    & & @5\degree & @10\degree & @20\degree & &\\
    \midrule
    satLoFTR & \checkmark
    & 32.39 & 46.73 & 59.17 & \textbf{44.34} & \textbf{79} \\
    satDualRC-Net & \checkmark
    & 11.21 & 20.59 & 33.75 & 25.40 & 51 \\
    SIFT + satCAPS  & \checkmark
    & 5.35 & 10.49 & 19.16 & 8.82 & 18 \\
    \midrule
    satLoFTR & \cross
    & 11.49 & 18.33 & 25.78 & 22.26 & 40 \\
    satDualRC-Net & \cross
    & 10.52 & 19.30 & 31.47 & 27.75 & 55 \\
    SIFT + satCAPS & \cross
    & 8.93 & 16.75 & 27.93 & 12.46 & 25 \\    
    \midrule
    LoFTR$\triangledown$ & \cross
    & \textbf{37.35} & \textbf{52.25} & \textbf{64.80} & 42.00 & 67 \\
    DualRC-Net$\triangledown$ & \cross
    & 8.79 & 16.42 & 27.58 & 24.26 & 49 \\
    SIFT + CAPS$\triangledown$ & \cross
    & 7.07 & 13.47 & 23.43 & 10.87 & 22 \\
    \bottomrule
\end{tabular}

==> tables/jax_matcher_performance_table.tex <==
\begin{tabular}{lcccccc}
    \toprule
    \multicolumn{7}{c}{\centering \textbf{Jacksonville}}\\
    \midrule
    \multirow{2}{1cm}[-.4em]{Method} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Rot.\\ Aug.\end{tabular}}
    & \multicolumn{3}{c}{Pose estimation AUC $\uparrow$} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}P $\uparrow$\\ \end{tabular}} %$\delta_{epi}\!=\!1$\end{tabular}} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}} N $\uparrow$\\\end{tabular}}\\
    \cmidrule(lr){3-5}
    & & @5\degree & @10\degree & @20\degree & &\\
    \midrule
    satLoFTR & \checkmark 
    & 65.52 & 78.94 & 87.27 & 54.96 & 108 
    \\
    satDualRC-Net & \checkmark 
    & 11.79 & 21.09 & 33.73 & 26.99 & 54 
    \\
    SIFT + satCAPS & \checkmark 
    & 8.00 & 15.16 & 26.43 & 11.15 & 22 
    \\
    \midrule
    satLoFTR & \cross 
    & \textbf{75.82} & \textbf{85.45} & \textbf{91.24} & \textbf{67.82} & \textbf{135} 
    \\
    satDualRC-Net & \cross 
    & 9.49 & 16.53 & 26.16 & 27.97 & 56 
    \\
    SIFT + satCAPS & \cross
    & 16.13 & 28.20 & 42.73 & 15.65 & 31 
    \\
    \midrule
    LoFTR$\triangledown$ & \cross 
    & 48.05 & 62.26 & 73.52 & 44.96 & 76 
    \\
    DualRC-Net$\triangledown$ & \cross 
    & 7.31 & 13.16 & 21.75 & 24.19 & 48 
    \\
    SIFT + CAPS$\triangledown$ & \cross 
    & 9.46 & 17.06 & 27.62 & 10.63 & 21 
    \\
    \bottomrule
\end{tabular}

==> tables/pipeline_comparison_table_main.tex <==
\begin{tabular}{ccccc}
    \toprule
    \textbf{Metric} & 
    \textbf{MAE} (m)$\downarrow$ &
    \textbf{RMSE} (m)$\downarrow$ &
    \textbf{Comp.} (\%) $\uparrow$
    \\ 
    \midrule
    JHU/APL\cite{bosch2017metric} & 0.47 & 2.20 & 64.1 \\ 
    RSP\cite{qin2016rpc} & 0.39 & 2.31 & 68.7 \\ 
    ASP\cite{nasa_ames} & 0.35 & 2.27 & 69.4 \\
    S2P\cite{Franchis_ISPRS14_S2P} & 0.37 & 2.59 & 73.2 \\ 
    \textbf{Our} & 0.59 & 2.38 & 70.53 \\
    \bottomrule
\end{tabular}

==> tables/pipeline_comparison_table_transpose.tex <==
\begin{tabular}{lccccc}
    \toprule
    & \textbf{Our} & S2P\cite{Franchis_ISPRS14_S2P} & JHU/APL\cite{bosch2017metric} & RSP\cite{qin2016rpc} & ASP\cite{nasa_ames} \\
    \midrule
    MAE (m)$\downarrow$ & 0.59 & 0.37 & 0.47 & 0.39 & 0.35 \\
    RMSE (m)$\downarrow$ & 2.38 & 2.59 & 2.20 & 2.31 & 2.27 \\
    Completeness (\%) $\uparrow$ & 70.53 & 73.2 & 64.1 & 68.7 & 69.4 \\
    \bottomrule
\end{tabular}


==> tables/simulated_rot/argentina_matcher_performance_table.tex <==
\begin{tabular}{cccccccc}
    \toprule
    \multicolumn{8}{c}{\centering \textbf{San Fernando}}\\
    \midrule
    \multirow{2}{*}{\rotatebox[origin=c]{90}{Config}}
    & \multirow{2}{1cm}[-.4em]{Method} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Rot.\\ Aug.\end{tabular}}
    & \multicolumn{3}{c}{Pose estimation AUC$\uparrow$} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Precision $\uparrow$\\ \end{tabular}} %$\delta_{epi}\!=\!1$\end{tabular}} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}} \# Matches $\uparrow$\\ ({\scriptsize{TP}})\end{tabular}}\\
    \cmidrule(lr){4-6}
    & & & @5\degree & @10\degree & @20\degree & &\\
    \midrule   
    % new
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Baseline}}
    & SIFT + CAPS\cite{Qianqian_ECCV20_CAPS} & \cross & 1.28 & 2.54 & 5.02 & 0.83 & 2 \\
    & DualRC-Net\cite{Li_NIPS20_DUALRC} & \cross & 2.85 & 4.84 & 8.71 & 1.72 & 3 \\
    & LoFTR\cite{Sun_CVPR21_LOFTR} & \cross & 10.33 & 14.89 & 18.63 & 1.60 & 1 \\
    & MatchFormer\cite{wang2022matchformer} & \cross & 48.93 & 54.19 & 58.78 & 7.15 & 13 \\
    \midrule
    \multirow{8}{*}{\rotatebox[origin=c]{90}{Trained on SatDepth}}
    & SIFT + satCAPS & \cross & 2.11 & 3.80 & 7.36 & 1.03 & 2 \\
    & satDualRC-Net & \cross & 2.70 & 5.22 & 10.01 & 1.75 & 4 \\
    & satLoFTR & \cross & 1.21 & 1.91 & 3.34 & 2.70 & 4 \\
    & satMatchFormer & \cross & 46.50 & 52.35 & 58.08 & 4.39 & 7 \\
    \cmidrule{2-8}
    & SIFT + satCAPS & \checkmark & 5.29 & 9.53 & 16.35 & 6.67 & 13 \\
    & satDualRC-Net & \checkmark & 12.56 & 23.24 & 36.61 & 15.58 & 31 \\
    & satLoFTR & \checkmark & 33.23 & 48.39 & 62.29 & 40.43 & 67 \\
    & satMatchFormer & \checkmark & 54.57 & 64.15 & 72.68 & 39.83 & 73 \\
    \bottomrule
\end{tabular}

==> tables/simulated_rot/jax_matcher_performance_table.tex <==
\begin{tabular}{cccccccc}
    \toprule
    \multicolumn{8}{c}{\centering \textbf{Jacksonville}}\\
    \midrule
    \multirow{2}{*}{\rotatebox[origin=c]{90}{Config}}
    & \multirow{2}{1cm}[-.4em]{Method} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Rot.\\ Aug.\end{tabular}}
    & \multicolumn{3}{c}{Pose estimation AUC$\uparrow$} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Precision $\uparrow$\\ \end{tabular}} %$\delta_{epi}\!=\!1$\end{tabular}} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}} \# Matches $\uparrow$\\ ({\scriptsize{TP}})\end{tabular}}\\
    \cmidrule(lr){4-6}
    & & & @5\degree & @10\degree & @20\degree & &\\
    \midrule    
    % new
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Baseline}}
    & SIFT + CAPS\cite{Qianqian_ECCV20_CAPS} & \cross & 1.30 & 2.34 & 4.20 & 0.41 & 1 \\
    & DualRC-Net\cite{Li_NIPS20_DUALRC} & \cross & 2.18 & 4.07 & 7.47 & 1.02 & 2 \\
    & LoFTR\cite{Sun_CVPR21_LOFTR} & \cross & 30.57 & 39.97 & 46.96 & 0.96 & 1 \\
    & MatchFormer\cite{wang2022matchformer} & \cross & 53.08 & 57.44 & 60.65 & 8.60 & 16 \\
    \midrule
    \multirow{8}{*}{\rotatebox[origin=c]{90}{Trained on SatDepth}}
    & SIFT + satCAPS & \cross & 2.67 & 4.63 & 7.66 & 1.05 & 2 \\
    & satDualRC-Net & \cross & 2.70 & 4.92 & 8.08 & 0.81 & 2 \\
    & satLoFTR & \cross & 17.24 & 21.94 & 25.80 & 35.24 & 60 \\
    & satMatchFormer & \cross & 86.15 & 92.05 & 95.43 & 69.44 & 139 \\
    \cmidrule{2-8}
    & SIFT + satCAPS & \checkmark & 7.51 & 13.46 & 23.00 & 10.12 & 20 \\
    & satDualRC-Net & \checkmark & 9.97 & 19.65 & 34.11 & 18.46 & 37 \\
    & satLoFTR & \checkmark & 65.12 & 78.61 & 86.78 & 54.70 & 106 \\
    & satMatchFormer & \checkmark & 81.37 & 89.01 & 93.56 & 61.96 & 124 \\
    \bottomrule
\end{tabular}

==> tables/simulated_rot/omaha_matcher_performance_table.tex <==
\begin{tabular}{cccccccc}
    \toprule
    \multicolumn{8}{c}{\centering \textbf{Omaha}}\\
    \midrule
    \multirow{2}{*}{\rotatebox[origin=c]{90}{Config}}
    & \multirow{2}{1cm}[-.4em]{Method} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Rot.\\ Aug.\end{tabular}}
    & \multicolumn{3}{c}{Pose estimation AUC$\uparrow$} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Precision $\uparrow$\\ \end{tabular}} %$\delta_{epi}\!=\!1$\end{tabular}} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}} \# Matches $\uparrow$\\ ({\scriptsize{TP}})\end{tabular}}\\
    \cmidrule(lr){4-6}
    & & & @5\degree & @10\degree & @20\degree & &\\
    \midrule    
    % 
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Baseline}} 
    & SIFT + CAPS\cite{Qianqian_ECCV20_CAPS} & \cross & 34.99 & 36.14 & 38.41 & 3.46 & 7 \\
    & DualRC-Net\cite{Li_NIPS20_DUALRC} & \cross & 35.50 & 37.84 & 41.37 & 8.46 & 17 \\
    & LoFTR\cite{Sun_CVPR21_LOFTR} & \cross & 47.52 & 52.44 & 56.45 & 17.29 & 16 \\
    & MatchFormer\cite{wang2022matchformer} & \cross & 86.10 & 90.23 & 93.20 & 53.95 & 107 \\
    \midrule
    \multirow{8}{*}{\rotatebox[origin=c]{90}{Trained on SatDepth}}  
    & SIFT + satCAPS & \cross & 35.44 & 37.56 & 40.94 & 5.43 & 11 \\
    & satDualRC-Net & \cross & 35.91 & 37.85 & 40.34 & 9.24 & 18 \\
    & satLoFTR & \cross & 36.31 & 37.71 & 39.48 & 8.02 & 12 \\
    & satMatchFormer & \cross & 83.24 & 87.97 & 91.56 & 50.11 & 99 \\
    \cmidrule{2-8}
    & SIFT + satCAPS & \checkmark & 37.33 & 41.29 & 47.09 & 8.65 & 17 \\
    & satDualRC-Net & \checkmark & 42.92 & 50.19 & 58.91 & 19.94 & 40 \\
    & satLoFTR & \checkmark & 63.53 & 72.88 & 80.70 & 43.53 & 82 \\
    & satMatchFormer & \checkmark & 81.83 & 86.65 & 90.49 & 44.10 & 86 \\
    \bottomrule
\end{tabular}

==> tables/simulated_rot/ucsd_matcher_performance_table.tex <==
\begin{tabular}{cccccccc}
    \toprule
    \multicolumn{8}{c}{\centering \textbf{UCSD}}\\
    \midrule
    \multirow{2}{*}{\rotatebox[origin=c]{90}{Config}}
    & \multirow{2}{1cm}[-.4em]{Method} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Rot.\\ Aug.\end{tabular}}
    & \multicolumn{3}{c}{Pose estimation AUC$\uparrow$} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}}Precision $\uparrow$\\ \end{tabular}} %$\delta_{epi}\!=\!1$\end{tabular}} 
    & \multirow{2}{*}[-.4em]{\begin{tabular}[c]{@{}c@{}} \# Matches $\uparrow$\\ ({\scriptsize{TP}})\end{tabular}}\\
    \cmidrule(lr){4-6}
    & & & @5\degree & @10\degree & @20\degree & &\\
    \midrule    
    % new
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Baseline}}
    & SIFT + CAPS\cite{Qianqian_ECCV20_CAPS} & \cross & 34.39 & 35.25 & 37.01 & 2.92 & 6 \\
    & DualRC-Net\cite{Li_NIPS20_DUALRC} & \cross & 36.22 & 38.30 & 41.35 & 8.76 & 18 \\
    & LoFTR\cite{Sun_CVPR21_LOFTR} & \cross & 47.88 & 52.88 & 57.00 & 18.78 & 13 \\
    & MatchFormer\cite{wang2022matchformer} & \cross & 88.12 & 92.41 & 95.25 & 64.23 & 128 \\
    \midrule
    \multirow{8}{*}{\rotatebox[origin=c]{90}{Trained on SatDepth}}
    & SIFT + satCAPS & \cross & 34.98 & 36.40 & 38.84 & 4.09 & 8 \\
    & satDualRC-Net & \cross & 36.11 & 38.32 & 41.25 & 9.02 & 18 \\
    & satLoFTR & \cross & 35.45 & 36.48 & 37.88 & 5.63 & 8 \\
    & satMatchFormer & \cross & 83.62 & 87.88 & 91.02 & 39.24 & 70 \\
    \cmidrule{2-8}
    & SIFT + satCAPS & \checkmark & 36.54 & 39.36 & 44.05 & 6.79 & 14 \\
    & satDualRC-Net & \checkmark & 42.06 & 48.33 & 56.24 & 16.86 & 34 \\
    & satLoFTR & \checkmark & 56.58 & 64.74 & 71.65 & 35.46 & 60 \\
    & satMatchFormer & \checkmark & 80.10 & 83.96 & 87.15 & 34.75 & 63 \\
    \bottomrule
\end{tabular}
